Spatial-Temporal Deep Intention Destination Networks for Online Travel Planning

Nowadays, artificial neural networks are widely used for users' online travel planning. Personalized travel planning has many real applications and is affected by various factors, such as transportation type, intention destination estimation, budget limit and crowdness prediction. Among those factors, users' intention destination prediction is an essential task in online travel platforms. The reason is that, the user may be interested in the travel plan only when the plan matches his real intention destination. Therefore, in this paper, we focus on predicting users' intention destinations in online travel platforms. In detail, we act as online travel platforms (such as Fliggy and Airbnb) to recommend travel plans for users, and the plan consists of various vacation items including hotel package, scenic packages and so on. Predicting the actual intention destination in travel planning is challenging. Firstly, users' intention destination is highly related to their travel status (e.g., planning for a trip or finishing a trip). Secondly, users' actions (e.g. clicking, searching) over different product types (e.g. train tickets, visa application) have different indications in destination prediction. Thirdly, users may mostly visit the travel platforms just before public holidays, and thus user behaviors in online travel platforms are more sparse, low-frequency and long-period. Therefore, we propose a Deep Multi-Sequences fused neural Networks (DMSN) to predict intention destinations from fused multi-behavior sequences. Real datasets are used to evaluate the performance of our proposed DMSN models. Experimental results indicate that the proposed DMSN models can achieve high intention destination prediction accuracy.

==> 0_OnlineExp.tex <==
\section{Online Experiment}
We deploy our model on Fliggy's online recommender platform, and conduct the experiments on standard A/B testing environment. The benchmark model is DIN, which has shown strongly competitive on CTR prediction task. The online evaluation metric is real-time CTR. 

\subsection{Online Results}
Table \ref{Table5} shows the average relative improvement results of CTR on each business line in one week.

\begin{table}[htbp]
  \caption{Average relative improvement results of CTR}\label{Table5}
  \centering
  \setlength{\tabcolsep}{2mm}{
  \begin{tabular}{l|c}
    \hline
     Business line & CTR \\
    \hline
    Train & +3.4\%\\
    Flight& +2.5\%\\
    Vacation items& +1.4\%\\
    Hotel& +1.4\%\\
    \hline
  \end{tabular}}
\end{table}

From Table \ref{Table5}, we observe that the proposed model DIN\&ATMC achieves significant CTR improvement on four business lines, and achieves highest CTR improvement on train ticket business line.

